Lightning: Scaling the GPU Programming Model Beyond a Single GPU

The GPU programming model is primarily aimed at the development of applications that run one GPU. However, this limits the scalability of GPU code to the capabilities of a single GPU in terms of compute power and memory capacity. To scale GPU applications further, a great engineering effort is typically required: work and data must be divided over multiple GPUs by hand, possibly in multiple nodes, and data must be manually spilled from GPU memory to higher-level memories. We present Lightning: a framework that follows the common GPU programming paradigm but enables scaling to large problems with ease. Lightning supports multi-GPU execution of GPU kernels, even across multiple nodes, and seamlessly spills data to higher-level memories (main memory and disk). Existing CUDA kernels can easily be adapted for use in Lightning, with data access annotations on these kernels allowing Lightning to infer their data requirements and the dependencies between subsequent kernel launches. Lightning efficiently distributes the work/data across GPUs and maximizes efficiency by overlapping scheduling, data movement, and kernel execution when possible. We present the design and implementation of Lightning, as well as experimental results on up to 32 GPUs for eight benchmarks and one real-world application. Evaluation shows excellent performance and scalability, such as a speedup of 57.2x over the CPU using Lighting with 16 GPUs over 4 nodes and 80 GB of data, far beyond the memory capacity of one GPU.

==> ppsections/motivation.tex <==
There are several 



Programming GPUs can be done using several techniques, but all follow a similar programming model  (e.g., CUDA, OpenCL, OneAPI, SYCL).
Since our work relies on NVIDIA CUDA, we use its work to explain several GPU concepts.

In GPU programming, the platform consists of a single \emph{host} process, running on the CPU, that controls one or more GPU \emph{devices}.
Each device has its own dedicated memory and data must be transferred explicitly between main memory and device memory.
The host coordinates manages this memory, by allocating memory and initiating data transfers, and submits work to be executed on the device.
Computation on the GPU is performed by submitting special GPU-specific functions (called \emph{kernels}) that are executed by a large number of GPU threads in parallel.
These threads are arranged in a 1-, 2-, or 3-dimensional rectangular grid where each thread maps to a 1-, 2-, or 3-dimensional index.
These threads are grouped into \emph{thread blocks}.
Threads within the same thread block can synchronize and communicate, while the thread blocks themselves run independent of each other and cannot synchronize with each other.

For a single GPU, the common workflow is straightforward: allocate buffer in device memory, transfer input data from host to device memory, submit a series of kernels to be executed, and, finally, transfer output data back to the host.
Howver, using just a single GPU presents limitations when scaling the application.
First and foremost, modern GPUs have just ${\sim}10{-}20$GB of memory, meaning large data sets cannot fit into memory of a single GPU.
Second, even though modern GPUs have an abundance of compute power, large problem sizes might still take hours or even days to process using a single high-end GPU.

In these scenarios, using multiple GPUs is an attractive solution, either by using multiple GPUs within one node or using cluster of GPU nodes.
However, this presents a large engineering effort for a multitude of reasons.

\begin{itemize}

\item
Instead of storing data in a single buffer, data must now be divided into chunks and distributed among the GPUs.
For some applications, it may even be beneficially to (partial) replicate data, for instance, storing a border of halo cells around each tile.

\item
Instead of launching a single kernel onto a single GPU, work most now also be split into chunks and distributed among the GPUs.
How work and data are distributed has an important impact on performance.

\item
When using a single GPU, it is often sufficient to submit a series of kernels onto a single compute stream and let the GPU perform scheduling.
However, when using multiple GPU, it is necessary to create multiple compute streams and manage dependencies by hand.

\item
When using a cluster, distributed computing concerns play a role such as communication libraries, serialization, flow-control, etc.

\end{itemize}



[Do we need more text here? This section is in a pretty rough state.]

